Credibility in Second-Price Auctions: An Experimental Test

We provide the first direct test of how the credibility of an auction format affects bidding behavior and final outcomes. To do so, we conduct a series of laboratory experiments where the role of the seller is played by a human subject who receives the revenue from the auction and who (depending on the treatment) has agency to determine the outcome of the auction. Contrary to theoretical predictions, we find that the non-credible second-price auction fails to converge to the first-price auction. We provide a behavioral explanation for our results based on sellers' aversion to rule-breaking, which is confirmed by an additional experiment.

==> Credible Auctions (EE revision)/misc.tex <==


We present a simple operationalization of the environment in \citet{akbarpour}.  An auction consists of:

\begin{itemize}
\item a finite set of agents: $N \cup \lbrace 0 \rbrace$, consisting of $\vert N \vert$ bidders and an auctioneer (player 0)
\bigskip
\item a set of outcomes: $X$, where an outcome $x = (y, t_N)$ consists of a winner $y \in N$ and a profile of payments $t_N \in \mathbb{R}^{\vert N \vert}$
\bigskip
\item a type space: $\Theta_N =  [\underline{v}, \overline{v}]^N$, which is governed by a joint probability distribution $D: \Theta_N \longrightarrow [0,1]$
\bigskip
\item agent utilities $u_i: X \times \Theta_N \longrightarrow \mathbb{R}$
\bigskip
\item a partition $\Omega_i$ of $X$ for each $i \in N$, which represents what agent $i$ directly observes about the outcome
\end{itemize}

We make several additional assumptions before taking the theory to the lab.  First, we restrict attention to auctions in which only the winner pays: $t_i = 0$ for $i \neq y$.  Second, we assume that bidders have private values and that the auctioneer desires revenue: $u_i ((y, t_N), \theta_N) = \mathbbm{1}_{i = y}(\theta_i) - t_i$ and $u_0 ((y, t_N), \theta_N) = \sum_{i \in N}t_i$.  Finally, we only allow each bidder to observe whether she wins the object and her own payment.  In other words, $(y, t_N), (y^\prime, t_N^\prime) \in \omega_i$ if and only if one of the following two conditions holds: (1) $y \neq i$ and $y^\prime \neq i$ or (2) $y = y^\prime = i$ and $t_i = t_i^\prime$.



==> misc.tex <==


We present a simple operationalization of the environment in \citet{akbarpour}.  An auction consists of:

\begin{itemize}
\item a finite set of agents: $N \cup \lbrace 0 \rbrace$, consisting of $\vert N \vert$ bidders and an auctioneer (player 0)
\bigskip
\item a set of outcomes: $X$, where an outcome $x = (y, t_N)$ consists of a winner $y \in N$ and a profile of payments $t_N \in \mathbb{R}^{\vert N \vert}$
\bigskip
\item a type space: $\Theta_N =  [\underline{v}, \overline{v}]^N$, which is governed by a joint probability distribution $D: \Theta_N \longrightarrow [0,1]$
\bigskip
\item agent utilities $u_i: X \times \Theta_N \longrightarrow \mathbb{R}$
\bigskip
\item a partition $\Omega_i$ of $X$ for each $i \in N$, which represents what agent $i$ directly observes about the outcome
\end{itemize}

We make several additional assumptions before taking the theory to the lab.  First, we restrict attention to auctions in which only the winner pays: $t_i = 0$ for $i \neq y$.  Second, we assume that bidders have private values and that the auctioneer desires revenue: $u_i ((y, t_N), \theta_N) = \mathbbm{1}_{i = y}(\theta_i) - t_i$ and $u_0 ((y, t_N), \theta_N) = \sum_{i \in N}t_i$.  Finally, we only allow each bidder to observe whether she wins the object and her own payment.  In other words, $(y, t_N), (y^\prime, t_N^\prime) \in \omega_i$ if and only if one of the following two conditions holds: (1) $y \neq i$ and $y^\prime \neq i$ or (2) $y = y^\prime = i$ and $t_i = t_i^\prime$.


